Interactive Proof Presentations with Cobra

We present Cobra, a modern proof presentation framework, leveraging cutting-edge presentation technology together with a state of the art interactive theorem prover to present formalized mathematics as active documents. Cobra provides both an easy way to present proofs and a novel approach to auditorium interaction. The presentation is checked live by the theorem prover, and moreover allows for live changes both by the presenter and the audience.

==> eptcsdata.tex <==
\providecommand{\firstpage}{43}
\providecommand{\publicationstatus}{Autexier, S. and Quaresma, P. (Eds.): Proceedings of 12th\\ International Workshop on User Interfaces for Theorem Provers (UITP 2016)\\
EPTCS 239, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.239.4}{10.4204/EPTCS.239.4}}
\pdfoutput=1

